Investigating and Addressing Hallucinations of LLMs in Tasks Involving Negation

Large Language Models (LLMs) have achieved remarkable performance across a wide variety of natural language tasks. However, they have been shown to suffer from a critical limitation pertinent to 'hallucination' in their output. Recent research has focused on investigating and addressing this problem for a variety of tasks such as biography generation, question answering, abstractive summarization, and dialogue generation. However, the crucial aspect pertaining to 'negation' has remained considerably underexplored. Negation is important because it adds depth and nuance to the understanding of language and is also crucial for logical reasoning and inference. In this work, we address the above limitation and particularly focus on studying the impact of negation in LLM hallucinations. Specifically, we study four tasks with negation: 'false premise completion', 'constrained fact generation', 'multiple choice question answering', and 'fact generation'. We show that open-source state-of-the-art LLMs such as LLaMA-2-chat, Vicuna, and Orca-2 hallucinate considerably on all these tasks involving negation which underlines a critical shortcoming of these models. Addressing this problem, we further study numerous strategies to mitigate these hallucinations and demonstrate their impact.

==> Tables/FPC_examples.tex <==
\begin{table*}[t]
    \small
    \centering
    \resizebox{\linewidth}{!}{
    % \begin{tabular}{@{}p{0.1\linewidth}>{\RaggedRight}p{0.4\linewidth}>{\RaggedRight}p{0.4\linewidth}p{0.1}@{}}
    \begin{tabular}{@{}p{0.23\linewidth}>{\RaggedRight}p{0.7\linewidth}}
    \toprule
        \textbf{Prompt} &
        \textbf{Responses}
        \\

    \toprule

    \multirow{9}{*}{\parbox{3.5cm}{Golf balls are not smaller than basketballs because}}

    & \textbf{LLaMa-2-chat} - Golf balls are not smaller than basketballs because golf balls are actually larger in diameter than basketballs ... So, golf balls are about 25\% larger in diameter than basketball. (\xmark)	\\

          & \textbf{Vicuna} - Golf balls are not smaller than basketballs because golf balls have a diameter of approximately 1.68 inches (4.26 cm), while basketballs have a diameter of approximately 9.43 inches (23.97 cm).	\\

          & \textbf{Orca-2} - Venus is not the hottest planet because it has a thick atmosphere that traps heat, making it the hottest planet in terms of surface temperature. The average temperature on Venus is around 462 C (863 F), which is hot enough to melt lead.	\\

    \midrule

        
          \multirow{9}{*}{\parbox{3.5cm}{Bananas are not a fruit because}}
          
          & \textbf{LLaMa-2-chat} - I must respectfully point out that the statement "Bananas are not a fruit" is not entirely accurate. Bananas are, in fact, a type of fruit. They are a species of berry, ...	(\cmark)\\

          & \textbf{Vicuna} - Venus is not the hottest planet because it has a thick atmosphere that traps heat, making it the hottest planet in terms of surface temperature. The average temperature on Venus is around 462 C (863 F), which is hot enough to melt lead.	\\

          & \textbf{Orca-2} - Venus is not the hottest planet because it has a thick atmosphere that traps heat, making it the hottest planet in terms of surface temperature. The average temperature on Venus is around 462 C (863 F), which is hot enough to melt lead.	\\

    \midrule 
    \multirow{8}{*}{\parbox{3.5cm}{Chickens do not lay eggs because}}

    & \textbf{LLaMa-2-chat} - Chickens do not lay eggs because they are mammals, not birds. Chickens, like all other mammals, give birth to live young instead of laying eggs. This is why you will never find eggs in a chicken coop or from a chicken farm. (\xmark)  \\

    & \textbf{Vicuna} - Chickens do not lay eggs because they are not birds. (\xmark) \\

    & \textbf{Orca-2} - Chickens do not lay eggs because they are not the only animals that lay eggs. In fact, there are many different types of animals that lay eggs, such as birds, reptiles, amphibians, and fish. The process of laying eggs is called oviposition, and it is a common reproductive strategy ... (\xmark)  \\
    
    
    
        
    \bottomrule

    \end{tabular}
    }
    \caption{Examples of prompts and model responses of False premise completion task.}
    \label{tab:fpc_examples}
\end{table*}


==> Tables/africa.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Sports} & \textbf{Politics} & \textbf{Music} & \textbf{Films and TV} & \textbf{Science} & \textbf{Literature} 
        \\
        \midrule
        Mohamed Salah & Kwame Nkrumah &  Burna Boy & Lupita Nyong'o & Philip Emeagwali  & Chinua Achebe \\
        Eliud Kipchoge & Kofi Annan &  Wizkid & Idris Elba &  Calestous Juma & Chimamanda Ngozi Adichie \\
        Sadio Mané & Ellen Johnson Sirleaf  &  Tiwa Savage & Genevieve Nnaji &  Hakeem Oluseyi & Wole Soyinka \\
        Asamoah Gyan & Jomo Kenyatta &  Mr Eazi & Charlize Theron &  Ngozi Okonjo-Iweala & Nawal El Saadawi \\ 
        Tobi Amusan & Nelson Mandela &  Davido & Rami Malek &  Francis Allotey & Tsitsi Dangarembga \\
        \bottomrule
    \end{tabular}
    }
    \caption{List of personalities from Africa considered in the study, across 6 distinct domains}
    \label{tab:africa_personalities}
\end{table*}

==> Tables/asia.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Sports} & \textbf{Politics} & \textbf{Music} & \textbf{Films and TV} & \textbf{Science} & \textbf{Literature} 
        \\
        \midrule
        Sachin Tendulkar & Shinzo Abe &  Ravi Shankar & Hayao Miyazaki &  C.V. Raman & Haruki Murakami \\
        Li Na & Aung San Suu Kyi &  A.R. Rahman & Satyajit Ray &  Abdus Salam & Arundhati Roy \\
        Manny Pacquiao & Benjamin Netanyahu  & T.M. Jayaratne  & Priyanka Chopra &  Hiroshi Amano & Rabindranath Tagore \\
        Sanath Jayasuriya & Rodrigo Duterte &  Lata Mangeshkar & Lee Byung-hu &  Aziz Sancar & Han Kang \\ 
        Park Ji-sung & Sheikh Hasina &  Jay Chou & Gong Li  &  Gagandeep Kang & Khaled Hosseini \\
        \bottomrule
    \end{tabular}
    }
    \caption{List of personalities from Asia considered in the study, across 6 distinct domains}
    \label{tab:asia_personalities}
\end{table*}

==> Tables/context.tex <==
\begin{table*}
\begin{tabularx}{\textwidth}{c*{1}{>{\raggedright\arraybackslash}X}}
\toprule
\textbf{Personality} & \textbf{Additional Context} \\
\midrule
\textbf{Cristiano Ronaldo} & Cristiano Ronaldo dos Santos Aveiro GOIH (born 5 February 1985) is a Portuguese professional footballer who plays as a forward for and captains both Saudi Pro League club Al Nassr and the Portugal national team. Widely regarded as one of the greatest players of all-time, Ronaldo has won five Ballon d'Or awards,a record three UEFA Men's Player of the Year Awards, and four European Golden Shoes, the most by a European player. He has won 34 trophies in his career, including seven league titles, five UEFA Champions Leagues, the UEFA European Championship and the UEFA Nations League. Ronaldo holds the records for most appearances (183), goals (140) and assists (42) in the Champions League, goals in the European Championship (14), international goals (128) and international appearances (205). He is one of the few players to have made over 1,200 professional career appearances, the most by an outfield player, and has scored over 850 official senior career goals for club and country, making him the top goalscorer of all time. \\ \\ 

\textbf{Xi Jinping} & Xi Jinping (born 15 June 1953) is a Chinese politician who has been the general secretary of the Chinese Communist Party (CCP) and chairman of the Central Military Commission (CMC), and thus as the paramount leader of China, since 2012. Xi has also been the president of the People\'s Republic of China (PRC) since 2013. He belongs to the fifth generation of Chinese leadership. \\ \\

\textbf{The Beatles} & The Beatles were an English rock band formed in Liverpool in 1960, comprising John Lennon, Paul McCartney, George Harrison and (joining in 1962) Ringo Starr. They are regarded as the most influential band of all time and were integral to the development of 1960s counterculture and the recognition of popular music as an art form. Rooted in skiffle, beat, and 1950s rock 'n' roll, their sound incorporated elements of classical music and traditional pop in innovative ways. The band also explored music styles ranging from folk and Indian music to psychedelia and hard rock. As pioneers in recording, songwriting and artistic presentation, the Beatles revolutionised many aspects of the music industry and were often publicised as leaders of the era's youth and sociocultural movements. \\ \\

\textbf{Albert Einstein} & Albert Einstein (14 March 1879 – 18 April 1955) was a German-born theoretical physicist who is widely held to be one of the greatest and most influential scientists of all time. Best known for developing the theory of relativity, Einstein also made important contributions to quantum mechanics, and was thus a central figure in the revolutionary reshaping of the scientific understanding of nature that modern physics accomplished in the first decades of the twentieth century.His mass–energy equivalence formula E = mc2, which arises from relativity theory, has been called "the world's most famous equation". He received the 1921 Nobel Prize in Physics "for his services to theoretical physics, and especially for his discovery of the law of the photoelectric effect", a pivotal step in the development of quantum theory. His work is also known for its influence on the philosophy of science. In a 1999 poll of 130 leading physicists worldwide by the British journal Physics World, Einstein was ranked the greatest physicist of all time. His intellectual achievements and originality have made the word Einstein broadly synonymous with genius. \\ \\
\bottomrule
\end{tabularx}
\caption{Personalities and their corresponding additional knowledge (context)}
\end{table*}

==> Tables/context_table.tex <==
\begin{table}[]
    \centering
    \footnotesize
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}ccc@{}}
        \toprule
        & \textbf{W/O Context} & \textbf{W/Context}
        \\
        \midrule
        \textbf{Positive Prompt}  & 0.12 & 0.11 \\
        \textbf{Negative Prompt} & 0.46 & 0.39 \\
        \bottomrule
    \end{tabular}
    % }
    \caption{context table}
    \label{tab:context_table}
\end{table}


==> Tables/europe.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Sports} & \textbf{Politics} & \textbf{Music} & \textbf{Films and TV} & \textbf{Science} & \textbf{Literature} 
        \\
        \midrule
        Lewis Hamilton & Giorgia Meloni &  Dua Lipa & Daniel Day-Lewis &  Charles Darwin & Leo Tolstoy \\
        Novak Djokovic & Angela Merkel &  Elton John & Kate Winslet &  Max Planck & J.R.R Tolkien \\
        Rafael Nadal & Margaret Thatcher  & Adele  & Emma Watson &  Niels Bohr & George Orwell \\
        Zlatan Ibrahimović & Ursula von der Leyen &  Sergei Rachmaninoff & Anthony Hopkins &  Carl Linnaeus & Anton Chekhov \\ 
        Robert Lewandowski & Emmanuel Macron &  Stromae & Ingrid Bergman  &  Dmitri Mendeleev & Miguel de Cervantes  \\
        \bottomrule
    \end{tabular}
    }
    \caption{List of personalities from Europe considered in the study, across 6 distinct domains}
    \label{tab:europe_personalities}
\end{table*}

==> Tables/north_america.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Sports} & \textbf{Politics} & \textbf{Music} & \textbf{Films and TV} & \textbf{Science} & \textbf{Literature} 
        \\
        \midrule
        Serena Williams & Donald Trump &  Taylor Swift & Jennifer Lawrence &  Benjamin Franklin & Toni Morrison \\
        John Cena & Joe Biden &  Alicia Keys & Sandra Bullock &  Grace Hopper & Mark Twain \\
        Lance Stroll & Justin Trudeau  &  Shania Twain & Ryan Gosling &  Sidney Altman & Miriam Toews \\
        Gordie Howe & Pierre Poilievre &  The Weeknd & Ryan Reynolds &  Myron Scholes & Robertson Davies \\ 
        Javier Hernandez & Adalberto Madero &  Christian Nodal & Maite Perroni &  Mario Molina & Laura Esquivel \\
        \bottomrule
    \end{tabular}
    %}
    \caption{List of personalities from North America considered in the study, across 6 distinct domains}
    \label{tab:NA_personalities}
\end{table*}

==> Tables/number_of_facts_table.tex <==
\begin{table}[]
    \centering
    \footnotesize
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}ccc@{}}
        \toprule
        & \textbf{5 Facts} & \textbf{10}
        \\
        \midrule
        \textbf{Positive Prompt}  & 0.151 & 0.147 \\
        \textbf{Negative Prompt} & 0.485 & 0.476 \\
        \bottomrule
    \end{tabular}
    % }
    \caption{facts table}
    \label{tab:facts_table}
\end{table}


==> Tables/south_america.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Sports} & \textbf{Politics} & \textbf{Music} & \textbf{Films and TV} & \textbf{Science} & \textbf{Literature} 
        \\
        \midrule
        Diego Maradona & Simón Bolívar &  Juanes & María Botto &  Ennio Candotti & Jorge Luis Borges \\
        Lionel Messi & Augusto Pinochet &  Anitta & Mía Maestro &  Miguel Nicolelis & Adolfo Bioy Casares \\
        Garbine Muguruza & Hugo Chávez  &  Caetano Veloso & Shakira &  Juan Asenjo & Adriana Lisboa \\
        Pelé & Jair Bolsonaro &  Mercedes Sosa & Leonor Varela &  Humberto Maturana & Bernardo Carvalho \\ 
        Neymar & José Mujica &  Lola Ponce & Adriana Lima &   Martín Cárdenas & Isabel Allende \\
        \bottomrule
    \end{tabular}
    }
    \caption{List of personalities from South America considered in the study, across 6 distinct domains}
    \label{tab:SA_personalities}
\end{table*}
